Tokenizing 3D Molecule Structure with Quantized Spherical Coordinates

The application of language models (LMs) to molecular structure generation using line notations such as SMILES and SELFIES has been well-established in the field of cheminformatics. However, extending these models to generate 3D molecular structures presents significant challenges. Two primary obstacles emerge: (1) the difficulty in designing a 3D line notation that ensures SE(3)-invariant atomic coordinates, and (2) the non-trivial task of tokenizing continuous coordinates for use in LMs, which inherently require discrete inputs. To address these challenges, we propose Mol-StrucTok, a novel method for tokenizing 3D molecular structures. Our approach comprises two key innovations: (1) We design a line notation for 3D molecules by extracting local atomic coordinates in a spherical coordinate system. This notation builds upon existing 2D line notations and remains agnostic to their specific forms, ensuring compatibility with various molecular representation schemes. (2) We employ a Vector Quantized Variational Autoencoder (VQ-VAE) to tokenize these coordinates, treating them as generation descriptors. To further enhance the representation, we incorporate neighborhood bond lengths and bond angles as understanding descriptors. Leveraging this tokenization framework, we train a GPT-2 style model for 3D molecular generation tasks. Results demonstrate strong performance with significantly faster generation speeds and competitive chemical stability compared to previous methods. Further, by integrating our learned discrete representations into Graphormer model for property prediction on QM9 dataset, Mol-StrucTok reveals consistent improvements across various molecular properties, underscoring the versatility and robustness of our approach.

==> chap/2_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

\textbf{Molecular Notation}.
A molecule is modeled as a graph $\gG = (\gV, \gE)$, where $\gV$ represents the set of atoms, and $\gE$ represents the set of chemical bonds between them. In addition to the molecular graph, we use $\gR$ to denote the conformation of $\gG$, forming a complete 3D molecular structure $\gM = (\gG, \gR) = (\gV, \gE, \gR)$. Each atom $v_i \in \gV$ is associated with a 3D spatial coordinate $\vx_i \in \mathbb{R}^3$, and its atom type is represented by $z_i \in \mathbb{Z}$, where $z_i$ is the atomic number (nuclear charge) of the $i$-th atom.

\subsection{Autoregressive Generation of 3D Molecules}
\label{subsec:prelim_arin3D}

In earlier tasks of 2D molecular graph generation, many works have modeled the problem in an autoregressive manner~\cite{popova2019molecularrnn,shi2020graphaf,luo2021graphdf}. They iteratively predicting new atom types and bond formations until no new atoms can be added or no bonds can be formed with the current molecule.
Similarly, autoregressive generation of 3D molecules follows a process where new atoms are sequentially placed in 3D space~\citep{simm2020reinforcement,luo2022gspherenet,zhang2023equivariant}. At the $i$-th step, denote the intermediate 3D molecular geometry generated from the preceding $i-1$ steps as $\gM_i = (\gG_i, \gR_i)$, consisting of $i$ atoms. This process can be described as constructing a sequence of increasingly larger fragments: $\gM = \{\gM_0, \gM_1, \dots, \gM_{|\gV|}\}$, where at step $i$, the $i$-th atom type $z_i$ and its spatial coordinates $\vx_i$ are generated. A local coordinate system is established at each stage $\gM_i$, predicting the atom's local coordinates, which are then transformed into global spatial coordinates. The process is divided into three main steps:
\begin{enumerate}[leftmargin=2em, topsep=0pt]
    \item \textit{Predict the atomic number}. Based on the partial molecular structure, the model predicts the next atom type $z_i$.
    \item \textit{Establish a local spherical coordinate system}. A coordinate system is defined by selecting three reference atoms. Typically, a focal atom $f$ is chosen, along with its closest and second-closest atoms, $c_1$ and $c_2$\footnote{Different approaches may vary slightly; for instance, in G-SphereNet~\citep{luo2022gspherenet}, $c_1$ is selected as the atom closest to $f$, and $c_2$ is the atom closest to $c_1$.}.
    \item \textit{Predict the new atom coordinates}. Conditioning on the spherical coordinate system, the model predicts the descriptors $d_i$, $\theta_i$, and $\phi_i$. Here, $d_i \in \sR^+$ is the distance between the new atom and $f$, while $\theta_i \in[0, \pi]$ and $\phi_i \in[0, 2\pi]$ are angular coordinates. Some later works, like~\citet{daigavane2024symphony}, avoid spherical coordinates in favor of orientation prediction to better handle symmetry.
\end{enumerate}
The order of the first and second steps can vary in some works~\citep{simm2020reinforcement}. 
Each step involves specific model predictions, described as follows: 
\begin{gather}
\begin{gathered}
z_i = f_z(\gM_{i-1}) \quad
p_f = f_p(\gM_{i-1}, z_i) \\
d_i   = f_d(\gM_{i-1}, p_f, z_i) \quad
\theta_i = f_\theta(\gM_{i-1}, p_f, z_i) \quad
\phi_i = f_\phi(\gM_{i-1}, p_f, z_i)
\end{gathered}
\end{gather}
In this work, the first two steps are deterministically defined based on line notation, removing the need for additional parametrized models. This approach distinguishes 3D line notation-based generation from existing autoregressive generation methods.

% \subsection{Vector Quantization}


% MolecularRNN, GraphAF, GraphDF
% G-SchNet, G-SphereNet, MolGym

% \subsection{3D Molecule Generation}
% % 3D分子生成主要有两条路，
% \subsection{Structure Tokenization}

